A Parameterized Family of Meta-Submodular Functions

Submodular function maximization has found a wealth of new applications in machine learning models during the past years. The related supermodular maximization models (submodular minimization) also offer an abundance of applications, but they appeared to be highly intractable even under simple cardinality constraints. Hence, while there are well-developed tools for maximizing a submodular function subject to a matroid constraint, there is much less work on the corresponding supermodular maximization problems. We give a broad parameterized family of monotone functions which includes submodular functions and a class of supermodular functions containing diversity functions. Functions in this parameterized family are called \emph{$\gamma$-meta-submodular}. We develop local search algorithms with approximation factors that depend only on the parameter $\gamma$. We show that the $\gamma$-meta-submodular families include well-known classes of functions such as meta-submodular functions ($\gamma=0$), metric diversity functions and proportionally submodular functions (both with $\gamma=1$), diversity functions based on negative-type distances or Jensen-Shannon divergence (both with $\gamma=2$), and $\sigma$-semi metric diversity functions ($\gamma = \sigma$).

==> MS_confApp3SemiMetric.tex <==
\section{Appendix: Semi-Metric Diversity \textcolor{red}{I think most of this was in the continuous paper so it may go.}}
\label{app:semimetric}

In this section, we establish the smoothness parameter associated with several of the discrete quadratic  functions discussed.
  In other words, we bound the approximate triangle inequality for their associated distance functions.

\begin{definition}
Let $d:[n]\times [n]\rightarrow \mathbb{R}_{\geq 0}$ be a distance function with the corresponding distance matrix $D\in \mathbb{R}^{n\times n}_{\geq 0}$ where $D_{a,b}=d(a,b)$. We say $d$ is a negative-type distance if for any $x\in \mathbb{R}^n$ with $||x||_1=0$ we have $x^{\top} Dx\leq 0$.
\end{definition}

\begin{proposition}
\label{prop:negtypeSemimetric}
Any negative-type distance $d:[n]\times [n]\rightarrow \mathbb{R}_{\geq 0}$ is $2$-semi-metric.
\end{proposition}
\begin{proof}%{Lemma~\ref{lemma:negtypeSemimetric}.}
Let $x=0.5e_a+0.5e_b-e_c$. We know
\begin{align*}
x^{\top} Dx & = 0.5d(a,b)-d(a,c)-d(b,c)   \leq 0.
\end{align*}
Therefore $d(a,b)\leq 2d(a,c)+2d(b,c)$ and $d$ is $2$-semi metric.
\end{proof}

Jensen-Shannon Divergence is a function which measures dissimilarity between probability distributions.
It is well-known that if $d$ is a JS measure, then  $\sqrt{d}$ is a metric. Hence JS distances form a $2$-semi-metric by the following result.


\begin{proposition}
\label{prop:sqrtdist}
Let $d:[n]\times [n]\rightarrow \mathbb{R}_{\geq 0}$ be a distance function such that $\sqrt{d(\cdot,\cdot)}$ is a metric. Then $d(\cdot,\cdot)$ is a  $2$-semi-metric.
\end{proposition}
\begin{proof}
By definition, we have 
\[
\sqrt{d(i,j)}\leq \sqrt{d(i,k)}+\sqrt{d(j,k)}.
\]
Therefore,
\[
d(i,j) \leq d(i,k) + d(j,k) + 2\sqrt{d(i,k) d(j,k)}.
\]
We also know that
\[
d(i,k) + d(j,k) - 2\sqrt{d(i,k) d(j,k)} = (\sqrt{d(i,k)}-\sqrt{d(j,k)})^2 \geq 0.
\]
Hence, 
\[
d(i,j) \leq 2(d(i,k) + d(j,k)).
\]
\end{proof}


\iffalse
\subsection{Second-Order-Modular Functions}
\label{app:subsecsemisecond}
In this section, we describe the structure of second-order-modular functions (defined by Korula et al.~\cite{KorulaMZ15}). We also discuss the smoothness parameter of quadratic functions defined on a $\sigma$-semi-metric distance. Moreover, we discuss the meta-submodularity parameter of the second-order-modular functions defined on a $\sigma$-semi-metric distance.

\begin{definition}[\cite{KorulaMZ15}]
A set functions $f:2^{[n]}\rightarrow\mathbb{R}$ is called second-order modular if $B_i(S\cup R)-B_i(S)=B_i(T\cup R)-B_i(T)$ for any $S\subseteq T$, $R\subseteq [n]\setminus T$, and $i\in [n]\setminus(T\cup R)$. 
\end{definition}

The following lemma characterize the structure of second-order modular functions. %The proof is included in Appendix~\ref{appendix1}.



\begin{lemma}
\label{lemma:2ndordermodular}
$f$ is a second-order modular function if and only if there exist symmetric $d:[n]\times [n]\rightarrow \mathbb{R}$, and $g:[n]\rightarrow\mathbb{R}$ such that
\[f(R) = \sum_{\{i,j\}\subset R}d(i,j)+\sum_{i\in R}g(i).\]
If $f$ is also supermodular (submodular), then $d$ is non-negative (non-positive).
\end{lemma}
\begin{proof}
Sufficiency is easy since
\begin{align*}
B_i(S\cup R)-B_i(S) & = (g(i)+\sum_{m\in S\cup R} d(m,i)) - (g(i)+\sum_{m\in S} d(m,i)) = \sum_{m\in R} d(m,i) \\ & = (g(i)+\sum_{m\in T\cup R} d(m,i)) - (g(i)+\sum_{m\in T} d(m,i)) \\ & =B_i(T\cup R)-B_i(T).
\end{align*}
To prove necessity, we first show  that if $i,j\in [n]$ and $S\subseteq [n]-i-j$ then, by second-order modularity
\[
B_j(S+i)-B_j(S)=B_j([n]-j)-B_j([n]-i-j),
\]
because $S \subseteq [n]-i$ ($[n]-i$ plays the role of $T$ in the definition of second-order modular). Now, let $d(i,j)=B_j([n]-j)-B_j([n]-i-j)$ and $g(i)=B_i(\emptyset)$. Note that $d$ is symmetric because
\begin{align*}
d(i,j) & = B_j([n]-j)-B_j([n]-i-j) = (f([n])-f([n]-j))-(f([n]-i)-f([n]-i-j)) \\ & =(f([n])-f([n]-i))-(f([n]-j)-f([n]-i-j))=B_i([n]-i)-B_i([n]-i-j)=d(j,i).
\end{align*}
For any $m$, let $R_m=\{v_1,\ldots,v_m\}$, and set $R_0=\emptyset$.
Consider a set $R=\{v_1,\ldots,v_r \}$. Then we have
\begin{align*}
f(R) & = \sum_{m=0}^{r-1} (f(R_m + v_{m+1})-f(R_m)) = \sum_{m=0}^{r-1} B_{v_{m+1}}(R_m) \\ & = \sum_{m=0}^{r-1} (\sum_{t=1}^{m} (B_{v_{m+1}}(R_t) - B_{v_{m+1}}(R_{t-1}))+B_{v_{m+1}}(R_0)) & \mbox{telescoping sum} \\ & = \sum_{m=0}^{r-1} (\sum_{t=1}^{m} (B_{v_{m+1}}([n]-v_{m+1}) - B_{v_{m+1}}([n]-v_t-v_{m+1}))+B_{v_{m+1}}(R_0)) \\ & = \sum_{m=0}^{r-1} \sum_{t=1}^{m} d(v_t,v_{m+1}) +\sum_{m=0}^{r-1} g(v_{m+1}).
\end{align*}
If $f$ is supermodular, $i,j\in [n]$, and $R\subseteq [n]-i-j$, we have
\[
f(R+i+j)-f(R+i)\geq f(R+j)-f(R).
\]
Therefore,
\[
g(j)+\sum_{v\in R+i} d(v,j)\geq g(j)+\sum_{v\in R} d(v,j),
\]
which means $d(i,j)\geq 0$. Similarly, if $f$ is submodular, $d$ is non-positive.
\end{proof}


\begin{proposition}
\label{prop:ossdiscretequad}
Let $A\in \mathbb{R}^{n\times n}$ be a symmetric, $0$-diagonal matrix. Let $b\in \mathbb{R}^n$ and $b\geq 0$. Then $F(x)=\frac{1}{2}x^{\top} A x + b^{\top} x$ is one-sided $2\sigma$-smooth if $A$ is $\sigma$-semi-metric.
\end{proposition}
\begin{proof}
Note that $\nabla^2 F(x) = A$ and $\nabla F(x) = Ax+b$. Therefore,
\begin{align*}
\sigma(\nabla_i F(x)+\nabla_j F(x)) & \geq \sigma(\sum_{k=1}^n A(i,k)x_k + \sum_{k=1}^n A(j,k)x_k) = \sum_{k=1}^n \sigma(A(i,k)+A(j,k))x_k \\ & \geq \sum_{k=1}^n A(i,j)x_k = ||x||_1 A(i,j) = ||x||_1 \nabla^2_{ij}F(x),
\end{align*}
where the first inequality follows from $b\geq0$ and the last inequality holds because $A$ is $\sigma$-semi-metric. Now by Lemma~\ref{lemma:probabilisticVersion}, we conclude that $F$ is one-sided $2\sigma$-smooth.

\iffalse
By Proposition~\ref{prop:semimetricmeta}, we know that $f(S)=\sum_{\{u,v\} \subseteq S} A(u,v) + \sum_{v \in S} b(v)$ is $\sigma$-meta-submodular. Moreover by Lemma~\ref{lem:2ndordermulti}, we know that $F$ is the multilinear extension of $f$. By meta-submodularity, for any $S\subseteq [n]$ and $i,j\in [n]$, we have
\[
|S|A_ij(S) \leq \sigma(B_i(S)+B_j(S)).
\]
Note that because of 2nd

First, let $F$ be one-sided $\sigma$-smooth and $i,j,k\in [n]$. Note that $\nabla^2 F(x) = A$ and $\nabla F(x) = Ax+b$. Set $u=\bm{e}_i+\bm{e}_j$ and $x=\bm{e}_k$. By the smoothness condition, we have
\[
2 A(i,j) \leq \sigma (\frac{2}{1})
\]
\fi
\end{proof}

\fi

